Dense Dynamics-Aware Reward Synthesis: Integrating Prior Experience with Demonstrations

Many continuous control problems can be formulated as sparse-reward reinforcement learning (RL) tasks. In principle, online RL methods can automatically explore the state space to solve each new task. However, discovering sequences of actions that lead to a non-zero reward becomes exponentially more difficult as the task horizon increases. Manually shaping rewards can accelerate learning for a fixed task, but it is an arduous process that must be repeated for each new environment. We introduce a systematic reward-shaping framework that distills the information contained in 1) a task-agnostic prior data set and 2) a small number of task-specific expert demonstrations, and then uses these priors to synthesize dense dynamics-aware rewards for the given task. This supervision substantially accelerates learning in our experiments, and we provide analysis demonstrating how the approach can effectively guide online learning agents to faraway goals.

==> abstract.tex <==
Many continuous control problems can be formulated as sparse-reward reinforcement learning (RL) tasks. In principle, online RL methods can automatically explore the state space to solve each new task. However, discovering sequences of actions that lead to a non-zero reward becomes exponentially more difficult as the task horizon increases. Manually shaping rewards can accelerate learning for a fixed task, but it is an arduous process that must be repeated for each new environment. We introduce a systematic reward-shaping framework that distills the information contained in $1)$ a task-agnostic prior data set and $2)$ a small number of task-specific expert demonstrations, and then uses these priors to synthesize dense dynamics-aware rewards for the given task. This supervision substantially accelerates learning in our experiments, and we provide analysis demonstrating how the approach can effectively guide online learning agents to faraway goals. 

==> acknowledgement.tex <==
This work was supported by the National Science Foundation under grant numbers 2409535 and 2214939, and also by the Office of Naval Research (ONR) under grant number N00014-22-1-2254.

==> analysis.tex <==
\begin{comment}
Following related analyses \cite{wang2023optimal, westenbroek2022lyapunov}, we derive our theoretical results under the simplifying assumption that the dynamics and policies are deterministic. In particular, we will use the map $f$ to denote the derterministic transition map $s' = f(s,a)$. Our analysis with focus on studying the effects of horizon shortening in our setting, and understanding 

\begin{equation}
V(s) = \gamma V(s') + r(s,\pi(s))
\end{equation}

\begin{equation}
\gamma V^\pi(s') - \gamma V^\pi(s) = (1-\gamma) V^\pi(s)
\end{equation}

\begin{equation}
\bar{V}^\pi(s_0) = \sum_{t=0}^{\infty} \gamma^t \bar{r}(s,a)
\end{equation}




\begin{prop}
Let ${\hat{\Phi} \colon \mathcal{S} \to \R}$ satisfy the following properties: $1)$ . Further assume that there exists $\pi \in \Pi$ such that if we apply the policy 
\end{prop}


\begin{equation}
\bar{V}(s) = \gamma \bar{V}(s') + \gamma \Phi(s') - \Phi(s) + r(s,a) 
\end{equation}

\begin{equation}
s
\end{equation}




\begin{equation}
A^\pi(s,a) = r(s,a) + \gamma V^\pi(s') - V(s)
\end{equation}
\begin{equation}
\bar{A}^\pi(s,a) = r(s,a) + \gamma \bar{V}^\pi(s') +\gamma \Phi(s') - \bar{V}(s) - \Phi(s).
\end{equation}
\end{comment}

==> figure_latex/heatmap_Lmaze.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/heatmap_Lmaze.pdf}
    \caption{Potential Heatmap for the Large Maze with Single Reset Grid}
    \label{fig:heatmap_Lmaze}
\end{figure}

==> figure_latex/heatmap_Lmaze_MReset.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/heatmap_Lmaze_MReset.pdf}
    \caption{Potential Heatmap for the Large Maze with Multiple Reset Grids}
    \label{fig:heatmap_Lmaze_MReset}
\end{figure}





==> figure_latex/heatmap_Mmaze.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/heatmap_Mmaze.pdf}
    \caption{Potential Heatmap for the Medium Maze with Single Reset Grid}
    \label{fig:heatmap_Mmaze}
\end{figure}

==> figure_latex/heatmap_maze.tex <==
\begin{figure*}[t!]
    \centering
    \subfigure[Medium maze]{\includegraphics[width=0.296\textwidth]{figures/heatmap_Mmaze.pdf}\label{fig:heatmap_Mmaze}}
    \subfigure[Large maze]{\includegraphics[width=0.34\textwidth]{figures/heatmap_Lmaze.pdf}\label{fig:heatmap_Lmaze}}
    \subfigure[Large maze with 3 reset grids]{\includegraphics[width=0.34\textwidth]{figures/heatmap_Lmaze_MReset.pdf}\label{fig:heatmap_Lmaze_MReset}}
    \vspace{-0.5em}
    \caption{\small{Potential heatmap for (a) medium maze with 1 reset grid, (b) large maze with 1 reset grid, and (c) large maze with 3 reset grids. 
    The agent constructs the $V_d^{j}(s_t^j) + \tilde{V}_g(s;s_j^t)$ in \eqref{eq:demo_pot} and \eqref{eq:sinle_pot} from a fixed state $s$ (green) and different demonstrated states (purple to yellow).
    The state chosen by the maximizations in \eqref{eq:sinle_pot} when constructing $\Phi$ is marked in pink.
    }}
    \vspace{-1.5em}
\label{fig:heatmap_mazes}
\end{figure*}

==> figure_latex/heatmap_push_grids.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/heatmap_push_grids.pdf}
    \caption{Potential Heatmap for the Push Slot with Multiple Reset Grids}
    \label{fig:heatmap_push_grids}
\end{figure}

==> figure_latex/render_heatmap_push.tex <==
% \begin{figure}[t!]
% \centering
% \begin{subfigure}[c]{0.2\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/render_push.png}
%     \caption{Pushing environment}
%     \label{fig:render_push}
% \end{subfigure}
% \hfill
% \begin{subfigure}[c]{0.29\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/heatmap_push_grids.pdf}
%     \caption{Potential heatmap}
%     \label{fig:heatmap_push_grids}
% \end{subfigure}
% \vspace{-1em}
% \caption{Push slot with 2 reset grids.}
% \vspace{-2em}
% \label{fig:render_heatmap_push}
% \end{figure}

% \begin{wrapfigure}{r}{0.5\textwidth}
% \subfigure[Pushing environment]{\includegraphics[width=0.25\textwidth]{figures/render_push.png}\label{fig:render_push}}
% \subfigure[Potential heatmap]{\includegraphics[width=0.35\textwidth]{figures/heatmap_push_grids.pdf}\label{fig:heatmap_push_grids}}
% \vspace{-1em}
% \caption{\small{Illustrative examples of push slot with 2 reset grids}}
% \vspace{-1em}
% \label{fig:render_heatmap_push}
% \end{wrapfigure}

% \begin{figure}[t!]
% \centering
% \subfigure[Pushing environment]{\includegraphics[width=0.25\textwidth]{figures/render_push.png}\label{fig:render_push}}
% \subfigure[Potential heatmap]{\includegraphics[width=0.35\textwidth]{figures/heatmap_push_grids.pdf}\label{fig:heatmap_push_grids}}
% \vspace{-1em}
% \caption{\small{Illustrative examples of push slot with 2 reset grids}}
% \vspace{-1em}
% \label{fig:render_heatmap_push}
% \end{figure}


==> intro_old.tex <==
\input{figure_latex/system_diagram}

Intelligent decision-making requires temporally extended reasoning across a multitude of environments. In principle, established exploration techniques for online deep reinforcement learning \cite{haarnoja2018soft,schulman2017proximal, chentanez2004intrinsically, bellemare2016unifying} can automatically achieve the spatial data coverage needed to successfully complete each new task. However, exploration for long-horizon tasks, especially those with sparse rewards, remains a significant bottleneck for these methods. In contrast, offline reinforcement learning attempts to bootstrap learning from diverse prior data sets \cite{kumar2020conservative, janner2021offline}. Yet, while both paradigms can benefit from amortizing learning across many tasks \cite{chane2021goal,andrychowicz2017hindsight}, solving novel long-horizon tasks remains challenging. 

In contrast, Learning from Demonstrations (LfD) frameworks can leverage expert trajectories to learn actions that are effective over long horizons but can struggle to obtain the necessary spatial data coverage needed to learn robust policies. This is due to the issue of compounding errors, wherein small differences in initial conditions or actions can cause rollouts to rapidly diverge from the expert training distribution \cite{ke2023ccil,ross2011reduction, block2023provable}. Thus, in order to obtain high-performance feedback policies, LfD techniques may require an impractical number of expensive-to-collect expert demonstrations \cite{ross2011reduction}. This challenge is compounded by low-quality or sub-optimal demonstrations, which degrade the performance of existing methods.

This paper introduces a novel reward-shaping framework that embraces the strengths of each of these learning paradigms. Our approach, which is depicted in Fig. \ref{fig:system_diagram}, combines broad prior experience with a handful of task-relevant expert demonstrations to synthesize dense dynamics-aware rewards that substantially accelerate online exploration and learning. Specifically, during an initial pre-training phase, our approach encodes information about the dynamics by learning a goal-conditioned value function from a prior task-agnostic data set. Then, given a small number of temporally extended demonstrations for a new task, we leverage the potential-based reward-shaping (PBRS) formalism \cite{ng1999policy} and construct a potential with two terms: $1)$ a term which incentivizes the agent to reach the nearest point on a demonstration, using the goal-conditioned value function to estimate the number of steps this will require and $2)$ a term encouraging the agent to follow the demonstration from this point to the task-specific goal. Altogether, the shaped reward provides dense supervision which biases the exploration of the online learner towards actions tracking nearby expert demonstrations to faraway goals. 

In summary, our approach leverages expert demonstrations for temporally extended reasoning, prior task-agnostic data to `fill the gaps' around the demonstrations with dense rewards, and a final online learning phase to smooth over potential deficiencies in these sources of data. Beyond massively accelerating learning, our approach has the following distinct benefits: 

% \textbf{Overcoming Sub-optimal Demonstrations and Dynamics Shift:} When using PBRS, the potential can be viewed as an approximation to the optimal value function of the original objective \cite{ng1999policy}. Crucially, while the reshaped reward can guide the exploration, the new objective preserves the optimal policies for the original problem. In our setting, when the demonstrations used to construct the potential are of poor quality, the potential will be a highly sub-optimal approximation to the value function. Similarly, when there is dynamics shift between the prior data set and the online learning environment, the goal-conditioned value functions may also be inaccurate in the new setting. Nonetheless, as our experiments demonstrate, in these scenarios, our approach still substantially accelerates learning while converging to optimal policies for the new task. 

% \textbf{Learning from (Partial) Observations:} In many practical scenarios, the agent may not have access to the actions taken by the expert, may only have access to partial state observations, and may even need to infer certain states from high-dimensional observations such as visual inputs. For example, when demonstrating how to push an object across a table, a human expert may elect to simply push the object with their own hand rather than turning to the burdensome process of teleoperation to generate rollouts that contain concrete actions for the robot. Our base reward-shaping approach only requires the states generated by the expert, and we demonstrate how the approach extends to situations with partial (and potentially high-dimensional) observations. However, because we implement our approach with off-policy RL, when actions are available, our approach benefits from including expert transitions in the replay buffer \cite{nair2018overcoming, rajeswaran2017learning}.
 
% \textbf{Shortening Learning Horizons:} During the initial pre-training phase, we focus on learning accurate goal-conditioned value estimates for goals which take a relatively small number of steps to reach (when compared with the temporally extended expert demonstrations incorporated downstream). Shortening the learning horizon enables us to effectively leverage tractable amounts of prior data while reusing it for many downstream tasks. We also investigate the effects of annealing the discount factor \cite{cheng2021heuristic} for the online learning agent with the reshaped objective. We show both theoretically and empirically how using a small discount factor early in training will cause the agent to greedily exploit the prior information baked into the dense rewards during initial exploration. Our experiments indicate this can further accelerate learning by a substantial margin. 

% We also investigate shortening the horizon for the online learning by annealing the discount factor during training \cite{cheng2021heuristic}
% We also demonstrate that, when certain theoretical conditions are met, our reshaped reward enables us to train agents online learning agents with subs
% We also demonstrate that our reshaped rewards enable us to decrease the discount factor for the online learning agent during initial phases 
% On the theoretical side, we demonstrate that when $1)$ these tubes cover the states encountered by the agent during the online training phase and $2)$ the goal-conditioned value estimates are reasonably accurate on the target domain, then our reshaped reward can still effectively guide the agent to the demonstrations when a much smaller discount factor is used (when compared to the original unshaped MDP). This enables us to anneal the discount factor during training, which causes the agent to greedily follow the potential early on while still obtaining optimal policies at convergence. We demonstrate that this approach can have a significant impact on training speed and stability in a number of domains.

\section{Related Work}

\textbf{Overcoming Distribution Shift in Imitation Learning:} A challenge for imitation learning is distribution shift, wherein small errors compound over time and cause the state distribution generated by the agent to diverge from that of the expert. Techniques such as DAGGER \cite{ross2011reduction} and DART \cite{laskey2017dart} use an interactive expert model to query expert trajectories that recover from mistakes made by the agent; however, this process may be overly arduous or impossible to implement in many practical scenarios. Frameworks such as GAIL \cite{ho2016generative}, SQIL \cite{reddy2019sqil}, and AIRL \cite{fu2017learning} allow the agent to interact with the environment independently and attempt to match the expert distribution over long horizons. The approach in \cite{reichlin2022back} learns a recovery policy which takes the agent back to the set of demonstrated states, but requires that the dynamics are known in the testing environment. Generative techniques such as \cite{ke2023ccil} use a learned model to perform data augmentation by generating actions returning the agent to the expert distribution. While these approaches are highly effective at imitating the expert, their performance is fundamentally limited by the quality of the demonstrations. 

\noindent\textbf{Reinforcement Learning with Demonstrations:} Most similar to our approach are techniques which use expert demonstrations to accelerate base off-policy reinforcement learning methods. Approaches such as \cite{nair2018overcoming, rajeswaran2017learning, hester2018deep} add demonstrations to replay buffers of base off-policy RL methods and use techniques such as prioritized experience replay and pre-training with behavior cloning to accelerate and stabilize learning. As we have demonstrated, these methods are directly compatible with our core reward-shaping technique. Other contributions have performed reward-shaping to guide agents back to demonstrated states \cite{brys2015reinforcement, zhao2023learning, pari2021surprising}, but rely on heuristic hand designed measures of the distance between a given state and a nearby demonstration (such as simple L2 distances). Our method bakes in prior knowledge about the dynamics into the reward which, as we discuss in Sec. \ref{sec:discounting}, is essential to accelerate learning. 


==> table_latex/median_success_rate.tex <==
\begin{table*}[ht]
  \centering
  \scriptsize
    \begin{tabular}{cccccccc}
    \toprule
    \multirow{2}{*}{Method} & Success Rate & \multicolumn{3}{c}{Maze} & \multicolumn{3}{c}{Push Slot} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}          & (\%)  & Medium 1 Grid & Large 1 Grid & Large 3 Grids & 1 Grid & 2 Grids & 1 Grid (Pointcloud) \\
    \midrule
    \midrule
    Buffer + Potential + Annealing & Q3 / Med. / Q1 & 100 / \textbf{100} / 100 & 100 / \textbf{100} / 100 & 100 / \textbf{100} / 99 & 100 / \textbf{100} / 99 & 98 / \textbf{96} / 85 & 97 / \textbf{95} / 94 \\
    \midrule
    Buffer + Potential & Q3 / Med. / Q1 & 100 / \textbf{100} / 100 & 100 / \textbf{100} / 100 &  87 / 78 / 56 & 100 / 99 / 99 & 97 / 95 / 94 & 96 / \textbf{95} / 94 \\
    \midrule
    Potential + Annealing & Q3 / Med. / Q1 & 100 / \textbf{100} / 100 & 100 / \textbf{100} / 100 & 100 / \textbf{100} / 99 & 99 / 98 / 24 & 97 / 94 / 88 & 97 / 94 / 93 \\
    \midrule
    Potential Only & Q3 / Med. / Q1 & 100 / \textbf{100} / 100 &  100 / 99 / 91 & 80 / 65 / 53 & 99 / 98 / 97 & 96 / 95 / 93 & 97 / \textbf{95} / 92 \\
    \midrule
    Buffer Only & Q3 / Med. / Q1 & 100 / \textbf{100} / 100 & 97 / 49 / 0 & 61 / 31 / 27 & 75 / 0 / 0 & 93 / 46 / 0 & 95 / 94 / 93 \\
    \midrule
    GAIL & Q3 / Med. / Q1 &  100 / \textbf{100} / 100  & 100 / 98 / 95  & 100 / 99 / 99 & 90 / 17 / 0 & 22 / 13 / 2 & 75 / 72 / 67 \\
    \midrule
    BC 1 Demo$^*$ & Q3 / Med. / Q1 & 38 / 28 / 18 & 37 / 34 / 30 & 25 / 20 / 16 & 1 / 0 / 0 & 1 / 0 / 0 & 0 / 0 / 0 \\
    \midrule
    BC 10 Demos & Q3 / Med. / Q1 & 57 / 48 / 46 & 74 / 69 / 65 & 77 / 68 / 64 & 47 / 35 / 26 & 16 / 12 / 9 & 0 / 0 / 0 \\
    \midrule
    BC 100 Demos & Q3 / Med. / Q1 & 100 / 99 / 98 & 100 / \textbf{100} / 99 & 100 / \textbf{100} / 99 & 54 / 51 / 48 & 26 / 23 / 17 & 1 / 0 / 0 \\
    \bottomrule
    \end{tabular}% 
  \caption{
    Median and quantiles of success rates. 
    The statistics are calculated over $10$ agents trained for the corresponding total environment steps (Tab. \ref{tab:env_para}).
    Our potential shaping approach results in more stable performance than the other baselines.
    ($^*$ For 2 and 3 reset grids, the same number of demonstrations are provided.)
  % Median and quantiles of success rate ($\%$) for all methods in the six tasks over $10$ seeds at corresponding total env steps. Our reward-shaping approach results in more stable performance than the baselines across random seeds.
  }
  \label{tab:mean_quant}
\end{table*}%
